Forbidden Patterns in Temporal Graphs Resulting from Encounters in a Corridor

In this paper, we study temporal graphs arising from mobility models, where vertices correspond to agents moving in space and edges appear each time two agents meet. We propose a rather natural one-dimensional model. If each pair of agents meets exactly once, we get a simple temporal clique where the edges are ordered according to meeting times. In order to characterize which temporal cliques can be obtained as such `mobility graphs', we introduce the notion of forbidden patterns in temporal graphs. Furthermore, using a classical result in combinatorics, we count the number of such mobility cliques for a given number of agents, and show that not every temporal clique resulting from the 1D model can be realized with agents moving with different constant speeds. For the analogous circular problem, where agents are moving along a circle, we provide a characterization via circular forbidden patterns. Our characterization in terms of forbidden patterns can be extended to the case where each edge appears at most once. We also study the problem where pairs of agents are allowed to cross each other several times, using an approach from automata theory. We observe that in this case, there is no finite set of forbidden patterns that characterize such temporal graphs and nevertheless give a linear-time algorithm to recognize temporal graphs arising from this model.

==> coverletter.tex <==

\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Computer and System Sciences

\bigskip

Dear Editors,

We are writing to submit our manuscript ``Forbidden Patterns in Temporal Graphs Resulting from Encounters in a Corridor'' to  \emph{Journal of Computer and System Sciences}.

Our manuscript studies \textbf{temporal graphs arising from mobility models}, where vertices correspond to agents moving in space and edges appear each time two agents meet. We mainly focus on the $1$-dimensional model, where agents move along a line.


  We characterize the temporal cliques that can be obtained as such `mobility graphs', for which we introduce the notion of forbidden patterns in temporal graphs.  We also provide a formula for the number of 1D mobility cliques for a given number of agents

An extended abstract containing the above results was published in the conference SSS 2023 (\textit{25th International Symposium on Stabilization, Safety, and Security of Distributed Systems}) under the same title. 

The current paper significantly extends this work of by providing the following new results:

  \begin{itemize}
    \item For the analogous circular problem, where agents are moving along a circle, we provide a characterization via circular forbidden patterns. %Our characterization in terms of forbidden patterns can be extended to the case where each edge appears at most once. 
    \item 
    We also study the problem where pairs of agents are allowed to cross each other several times, using an approach from automata theory. We observe that in this case, there is no finite set of forbidden patterns that characterize such temporal graphs and nevertheless give a linear-time algorithm to recognize temporal graphs arising from this model.
    \item Finally, we show that not every temporal clique resulting from the 1D model can be realized with agents moving with different constant speeds.

  \end{itemize}




Our submission has the following keywords: temporal graphs, mobility models, forbidden patterns, mobile clique.

We suggest \textbf{Paola Flocchini} as an associate editor for our submission.



We confirm that none of the co-authors listed below have a conflict of interest with the  editor we suggest above. Further, we confirm that all co-authors below consent to the submission of this manuscript to  \emph{Journal of Computer and System Sciences}.

\bigskip

Sincerely,

\bigskip

M\'onika Csik\'os (Universit\'e Paris Cit\'e)\\
Michel Habib (Universit\'e Paris Cit\'e)\\
Minh-Hang Nguyen (Universit\'e Paris Cit\'e)\\
Mikaël Rabie (Universit\'e Paris Cit\'e)\\
Laurent Viennot (INRIA Paris)


\end{document}








































